The descriptive complexity approach to LOGCFL

Building upon the known generalized-quantifier-based first-order characterization of LOGCFL, we lay the groundwork for a deeper investigation. Specifically, we examine subclasses of LOGCFL arising from varying the arity and nesting of groupoidal quantifiers. Our work extends the elaborate theory relating monoidal quantifiers to NC1 and its subclasses. In the absence of the BIT predicate, we resolve the main issues: we show in particular that no single outermost unary groupoidal quantifier with FO can capture all the context-free languages, and we obtain the surprising result that a variant of Greibach's ``hardest context-free language'' is LOGCFL-complete under quantifier-free BIT-free projections. We then prove that FO with unary groupoidal quantifiers is strictly more expressive with the BIT predicate than without. Considering a particular groupoidal quantifier, we prove that first-order logic with majority of pairs is strictly more expressive than first-order with majority of individuals. As a technical tool of independent interest, we define the notion of an aperiodic nondeterministic finite automaton and prove that FO translations are precisely the mappings computed by single-valued aperiodic nondeterministic finite transducers.

==> macros2e97.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% Sectioning
% 



% sections:
% 

\makeatletter
\renewcommand{\section}{\@startsection
	{section}%
	{1}%
	{0mm}%
	{-2\baselineskip}%
	{\baselineskip}%
	{\normalfont\large\bf}}
\renewcommand{\subsection}{\@startsection
	{subsection}%
	{1}%
	{0mm}%
	{-2\baselineskip}%
	{\baselineskip}%
	{\normalfont\normalsize\bf}}
\makeatother
	


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% Theorem environments and the like

% diverse layout changes
\makeatletter
\def\@begintheorem#1#2{\parskip0pt plus3pt\it \trivlist \item[\hskip 
\labelsep{\bf #1\ #2.}]}
\def\@opargbegintheorem#1#2#3{\parskip0pt plus3pt\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ #3.}]}
\makeatother


% Environments with Text in Roman
% i.e.: Definitions

\makeatletter

\def\newdefinition#1{\@ifnextchar[{\@odefi{#1}}{\@ndefi{#1}}}

\def\@ndefi#1#2{%
\@ifnextchar[{\@xndefi{#1}{#2}}{\@yndefi{#1}{#2}}}

\def\@xndefi#1#2[#3]{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}\@addtoreset{#1}{#3}%
\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
  \csname the#3\endcsname \@deficountersep \@deficounter{#1}}%
\global\@namedef{#1}{\@defi{#1}{#2}}\global\@namedef{end#1}{\@enddefi}}}

\def\@yndefi#1#2{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@deficounter{#1}}%
\global\@namedef{#1}{\@defi{#1}{#2}}\global\@namedef{end#1}{\@enddefi}}}

\def\@odefi#1[#2]#3{\expandafter\@ifdefinable\csname #1\endcsname
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
\global\@namedef{#1}{\@defi{#2}{#3}}%
\global\@namedef{end#1}{\@enddefi}}}

\def\@defi#1#2{\refstepcounter
    {#1}\@ifnextchar[{\@ydefi{#1}{#2}}{\@xdefi{#1}{#2}}}

\def\@xdefi#1#2{\@begindefi{#2}{\csname the#1\endcsname}\ignorespaces}
\def\@ydefi#1#2[#3]{\@opargbegindefi{#2}{\csname
       the#1\endcsname}{#3}\ignorespaces}

\def\@deficounter#1{\noexpand\arabic{#1}}
\def\@deficountersep{.}
%deleted September 2, 1986 MDK
%\def\@makethmnumber#1#2{\bf #1 #2:}
\def\@begindefi#1#2{\it \trivlist \item[\hskip \labelsep{\bf #1\ #2.}]\rm}
\def\@opargbegindefi#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ #3.}]\rm}
\def\@enddefi{\endtrivlist}

\makeatother


%
% Environment-Vereinbarungen:

\newtheorem{thm}{Theorem}[section]
\newtheorem{coro}[thm]{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{propo}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}

\newtheorem{question}{Open Question}

\newdefinition{defi}[thm]{Definition}
\newdefinition{example}[thm]{Example}
\newdefinition{problem}[thm]{Problem}
\newdefinition{remark}[thm]{Remark}

% proof environment
%\newcommand\qedsymbol{\ding{113}}
\newcommand\qedsymbol{$\square$}
\def\endproof{{\unskip\nobreak\hfil\penalty50
		      \hskip1em\hbox{}\nobreak\qedsymbol
		      \parfillskip=0pt\par\endtrivlist\addpenalty{-100}}} 
\def\proof{\trivlist
	\penum=1%penum: siehe unten!
	\item[\hskip \labelsep{\it Proof.}]}

\def\endoutline{{\unskip\nobreak\hfil\penalty50
		      \hskip1em\hbox{}\nobreak\qedsymbol
		      \parfillskip=0pt\par\endtrivlist\addpenalty{-100}}} 
\def\outline{\trivlist
	\penum=1%penum: siehe unten!
	\item[\hskip \labelsep{\it Proof sketch.}]}

% eigenes enumerate fuer Beweise, um Platz zu sparen ...
\newcount\penum
\def\pitem{\ifnum\penum>1\par\fi\the\penum. \advance\penum by1}


% numerierte Gleichungen, Bemerkungen, etc; 
% nur mit Nummer, ohne "Satz", "Korollar", ...

\newenvironment{eqn}
	{\trivlist\refstepcounter{thm}\item[\hskip \labelsep{\bf \thethm.}]}
	{\endtrivlist}



\newcounter{noheadsectionctr}[section]
\def\noheadsection{\addtocounter{noheadsectionctr}{1}
	\par\noindent{\bf\arabic{section}.\arabic{noheadsectionctr}. }}



\newcommand\todo[1]{\par{\sl #1}}
\newcommand\marg[1]{\marginpar{\raggedright\footnotesize\sl #1}}



